Spatial distribution of graffiti: A complex network approach

Despite the great differences among cities, they face similar challenges regarding social inequality, politics and criminality. Urban art express these feelings from the citizen point-of-view. In particular, the drawing and painting of public surfaces may carry rich information about the time and region it was made. Existing studies have explored the spatial distribution of graffiti, but most of them considered graffiti as a whole, with no separation among the types. Also, the analyses rarely take into account the city topology. In this work, we propose to categorize the graffiti into three types: simple scribbles, complex scribbles, canvases. We analyze the spatial distribution and identify the spatial bias of each type. To further analyze the spatial distribution of the types, we apply concepts from complex networks. First, regions (communities) defined by the connectivity profiles of the city network are obtained and the prevalence of each type of graffiti over these regions are analyzed. Next, a measure based on the dynamics of the network (accessibility) is calculated and compared to the distribution of the graffiti types. A case study is performed in the analysis of three different categories of graffiti in the city of Sao Paulo, Brazil. The results showed that the categories present characteristic spatial distributions. The ratio of each type per community of the network, though, does not pose significant deviations. Finally, a small positive correlation was observed between the locations of each graffiti type and the accessibility.

==> abstract.tex <==
Graffiti are commonly found in many cities around the world. Their study is important for several reasons, including a better understanding of underlying social dynamics, correlations with socioeconomic indices, content, among other possibilities. In this work, we address the problem of graffiti spatial and topological distribution by using a combination of different approaches, with emphasis on pattern recognition and network science. The focus of interest is on the identification of graffiti groups based on their visual properties, allowing the study of their spatial and topological distribution in city spaces, especially regarding their modular structure (communities). The developed methodology involves: (i) obtaining a significant number of graffiti samples; (ii) clustering these graffiti into major groups; (iii) obtaining the spatial distribution of each of the graffiti in the city space (taking into account the respective geographical coordinates). The latter data provides the means for verifying if graffiti of the same type tend to appear topologically near one another, or following some other spatial arrangement such as concentrating on some administrative zone or communities of the network defined by the streets of the considered city.


==> acknowledgments.tex <==
\section{Acknowledgments} 
\label{sec:acknowledgments}
The authors would like to thank FAPESP (\#2019/01077-3, \#2015/22308-2, \#2019/16223-5, and \#2018/10489-0), CAPES and CNPQ.



==> conclusion.tex <==
\section{Conclusion} 
\label{sec:conclusion}
Graffiti has long been studied as a human expression phenomenon. Visually it can be associated with very different visual forms. No studies up to date have focused on the geographical distribution of visual forms of graffiti and its relationship with the formation of network communities. In this work, we established three different visual forms of graffiti and analyzed a city regarding the distribution of these forms. We compare this distribution to the local distribution inside the communities obtained from the topology. Results indicate that within the data analyzed, no associations can be found between the communities and the distribution of each type of graffiti.


==> introduction.tex <==
\section{Introduction} 
\label{sec:introduction}

% The writing on public surfaces is commonly known as \emph{graffiti} and it is often done in an unauthorized way. Governments invariably spend large sums of money to contain these acts~\cite{wilson1982broken}. Like it or not, graffiti is part of the scenery of most major cities in the world and as such, this urban phenomenon has been widely studied in different fields, including sociology, criminology, urbanism and visual art~\cite{lachmann1988graffiti,ferrell1993crimes,ferrell1995urban}.
The writing on public surfaces is commonly known as \emph{graffiti}, which is often done in an unauthorized way. Governments invariably spend large sums of money to contain these acts~\cite{wilson1982broken}. Like it or not, graffiti is part of the scenery of most major cities in the world, and as such, this urban phenomenon has been widely studied in different fields, including sociology, criminology, urbanism, and visual art~\cite{lachmann1988graffiti,ferrell1993crimes,ferrell1995urban}.

The spread of graffiti is most notorious in urban environments. One of the reasons is related to the visibility gained by painting \emph{canvases} in well-localized streets compared to rural areas. Furthermore, the city is also an object of constant research, and in particular, the application of mathematical models to cities has shown several interesting results~\cite{batty2007cities,barthelemy2011spatial,bettencourt2013origins}. Among the aspects that can differentiate between cities, topology and community detection have been often considered~\cite{costa2007characterization,barthelemy2011spatial}. Several approaches that tackle the problem of community detection~\cite{fortunato2010community} but~\cite{rosvall2008maps} have (tem algum problema com esta sentenca???: Eric, pode corrigir?) shown to be a highly stable and fast community detection approach. It approaches the problem by compressing the information of a random walk on the network implemented with the use of greedy search and simulated annealing.

One question that may arise is whether the communities of the city privilege specific types of graffiti over others. Especially what are the impacts of the existence of communities in a network and the distribution of types of graffiti within them. There are no works to \textcolor{red}{the best of} our knowledge that studied this particular question.

In this work, we propose to investigate the relationship between the network communities and the distribution of graffiti within each community. First, a random sample of the graffiti of a city is categorized into three visual types, and the relative distribution of each type is calculated. The communities of the same city are obtained, and the distribution of each type of graffiti inside each region is compared to the city distribution.  These procedures have been applied using data from a Brazilian city popularly known for containing many areas affected by graffiti -- \emph{São Paulo}. The results using these data showed little impact of the communities over the distribution of each type of graffiti inside each region.

This text is divided as follows: in Section~\ref{sec:methods}, the data, and tools developed are explained; in Section~\ref{sec:results}, the results are presented and discussed and in Section~\ref{sec:conclusion} the conclusions, as well as the limitations of our approach, are presented.


==> methods.tex <==
\section{Materials and methods} 
\label{sec:methods}

% The data utilized in this work are the same as utilized in~\cite{tokuda2019quantifying}. Data consists of images from~\cite{googlemaps}, which were obtained in different weather conditions, times and with dense coverage.
Here, we employed the same data as we used in~\cite{tokuda2019quantifying}, which consists of images from~\cite{googlemaps}, obtained in different weather conditions, times, and with dense coverage.

% The first step consists of selecting a random sample of the images of the region of interest. The initial triage filters the images that do are not affected by graffiti. Among the occurrences of graffiti, three forms are considered: simple scribbles (type A), filled words (type B) and paintings and textures (types C). Please refer to Figure~\ref{fig:graffititypes} for a sample of each type of graffiti considered. The overall count of graffiti in the sample is obtained and the ratio of each type is calculated.
The first step consists of selecting a random sample of the images of the region of interest. The initial triage filters the images that do are not affected by graffiti. Among the occurrences of graffiti, three forms are considered: simple scribbles (type A), filled words (type B) and paintings, and textures (types C). Figure~\ref{fig:graffititypes} illustrates the considered graffiti types. The overall counts of each type are obtained {from a visual inspection}, and the ratios are calculated.

\begin{figure}[ht!]
    \begin{subfigure}[b]{0.3\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{img/IMG_20180705_084738544_HDR_type1}
	\caption{Type A}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
	    \centering
	\includegraphics[width=\textwidth]{img/IMG_20180705_084955051_HDR_type2}
	\caption{Type B}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
	    \centering
	\includegraphics[width=\textwidth]{img/batman01_type3}
	\caption{Type C}
    \end{subfigure}

    \caption{Categories of graffiti considered in this work. 
    %Images from personal collection.
    {These images were taken from personal collection.}}
    \label{fig:graffititypes}
\end{figure}

The communities are identified using Infomap algorithm~\cite{rosvall2008maps} and the count is compared to the overall count. A normalization step is considered in this step to allow a comparison of regions of different areas. In particular, the overall counts are normalized by the convex polygon delimited by each community. Finally, the ratio of each type inside each community is compared to the overall ratio.


==> results.tex <==
\section{Results} 
\label{sec:results}

% The street network of São Paulo was obtained from~\cite{openstreetmap}. The network is a directed graph composed of 112,014 nodes and 287,592 links. The streets network does not cover the city in its entirety mainly due to the natural and population characteristics of the southern regions (please refer to the map on the right of Figure~\ref{fig:mapcomm}).
In this study, we considered the street network of São Paulo, obtained from~\cite{openstreetmap}, which is directed and composed of 112,014 nodes and 287,592 links. This type of network does not cover the city in its entirety, mainly due to the natural and population characteristics of the southern regions (please refer to the map on the right of Figure~\ref{fig:mapcomm}). 
 
% A random sample of 8,003 images from~\cite{googlemaps} was initially obtained and manually annotated. A total of 1,187 graffiti images were identified, which have been categorized into types A, B, and C with count 837, 145 and 204 each, respectively. The location and the types are shown in Figure~\ref{fig:maptypes}. These results indicate that approximately 14.5\% of the street views of this city contains at least a mark of graffiti, with an approximately 71\%-12\%-17\% composition of types A, B, and C respectively.
A random sample of 8,003 images of~\cite{googlemaps} was initially obtained and manually annotated. A total of 1,187 graffiti images were identified, which have been categorized into three types A, B, and C, with  837, 145, and 204 pictures, respectively. The locations and the types are shown in Figure~\ref{fig:maptypes}. These results indicate that approximately 14.5\% of the street views contain at least a mark of graffiti, with an approximately 71\%-12\%-17\% composition of types A, B, and C, respectively.

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.28\textwidth]{img/map_types.png}
	\caption{Location of each type of graffiti in the city.}
	\label{fig:maptypes}
\end{figure}

% The communities were identified in this network resulting in 6 communities, as can be seen on the right of Figure~\ref{fig:mapcomm}. The total number of occurrences of graffiti in each region defined by the communities is shown on the left of Figure~\ref{fig:overallcount}. Despite there is a high number of occurrences in the community C2, the highest \emph{density} of graffiti appears in the community C4, as can be seen in the normalized counts on the same figure.
The measured number of network communities is 6, as can be seen on the right-hand side of Figure~\ref{fig:mapcomm}. The graffiti counts of the communities are displayed on the left of Figure~\ref{fig:overallcount}. Despite there is a high number of occurrences in the community C2, the highest \emph{density} of graffiti was found to be in the community C4, as can be seen in the normalized counts on the same figure.

% The composition by types of graffiti in each community is shown in the charts of Figure~\ref{fig:typescount}. /Each chart compares the ratios of one type of graffiti within the communities and the dashed vertical line represents the overall ratio of that type of graffiti. For instance, we notice that within the occurrences within the community C5, 74\% of the occurrences of graffiti are of type A, 9\% of type B and 16\% of type C. Compared to the overall ratios, this region presents a higher presence of type A while having less presence of type B. Despite the deviations found, the results indicate that there are no significant variations on the proportions of each type of graffiti induced by the communities.
The composition by types of graffiti respectively to each community is shown in the charts of Figure~\ref{fig:typescount}. Each chart compares the ratios of one type of graffiti within the communities, and the dashed vertical line represents the overall ratio of that type of graffiti. For instance, within the occurrences in the community C5, 74\% of the occurrences of graffiti are of type A, 9\% of type B, and 16\% of type C. Compared to the overall ratios, this region presents the highest presence of type A while having the lowest presence of type B. Despite the deviations found, the results indicate that there are no significant variations on the proportions of each type of graffiti induced by the communities.

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.28\textwidth]{img/map_comm.png}
	\caption{Network communities obtained using~\cite{rosvall2008maps}.}
	\label{fig:mapcomm}
\end{figure}

\begin{minipage}[b]{0.95\textwidth}
\begin{minipage}[b]{0.2\textwidth}
	\centering
	\small
	\begin{tabular}[b]{lr}
		\toprule
		Community& count\\ \midrule
		C1 & 242\\
		C2 & 287\\
		C3 & 249\\
		C4 & 195\\
		C5 & 149\\
		C6 & 65\\
		\bottomrule
	\end{tabular}
	\vspace{1em}
\end{minipage}
\hfill
\begin{minipage}[b]{0.7\textwidth}
	\centering
	\includegraphics[width=\textwidth]{img/countsnormalized.pdf}
\end{minipage}
	\captionof{figure}{Comparison of the overall count of graffiti in each community. The absolute count is shown on the table on the left while the normalized count by the area is shown on the right.}
	\label{fig:overallcount}
\end{minipage}

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.98\textwidth]{img/count_per_type.pdf}
	\caption{Ratio of each type of graffiti by community. The vertical dashed lines represents the ratio of each type of graffiti in the entire city.}
	\label{fig:typescount}
\end{figure}


